HOTCAKE: Higher Order Tucker Articulated Kernels for Deeper CNN Compression

The emerging edge computing has promoted immense interests in compacting a neural network without sacrificing much accuracy. In this regard, low-rank tensor decomposition constitutes a powerful tool to compress convolutional neural networks (CNNs) by decomposing the 4-way kernel tensor into multi-stage smaller ones. Building on top of Tucker-2 decomposition, we propose a generalized Higher Order Tucker Articulated Kernels (HOTCAKE) scheme comprising four steps: input channel decomposition, guided Tucker rank selection, higher order Tucker decomposition and fine-tuning. By subjecting each CONV layer to HOTCAKE, a highly compressed CNN model with graceful accuracy trade-off is obtained. Experiments show HOTCAKE can compress even pre-compressed models and produce state-of-the-art lightweight networks.

==> Chapters/old_experiments.tex <==
%--------------------
% layer-wise VGG-16
%--------------------



% \begin{table}[t]\scriptsize
% \caption{Caption}
% \scriptsize
% \centering
% \begin{tabular}{cccccccc}
% \noalign{\hrule height 0.75pt}
% CONV layer & 4 & 5 & 6 & 7 & 9 & 12 & Total \\
% \hline
% Origin & $74$K & $295$K & $1180$K & $4719$K & $1180$K & $885$K & $8333$K\\
% Tucker-2 & $51$K & $201$K & $795$K & $3405$K & $660$K & $564$K & $5736$K \\
% HOTCAKE & $22$K & $89$K & $352$K & $1548$K & $305$K & $250$K & $2566$K\\
% \tabincell{c}{Compression\\ Ratio} & \tabincell{c}{$3.36 \times$\\ $(2.32 \times)$} & \tabincell{c}{$3.31 \times$\\ $(2.26 \times)$} & \tabincell{c}{$3.35 \times$\\ $(2.26 \times)$} & \tabincell{c}{$3.05 \times$\\ $(2.24 \times)$} & \tabincell{c}{$3.87 \times$\\ $(2.16 \times)$} & \tabincell{c}{$3.54 \times$\\ $(2.26 \times)$} & \tabincell{c}{$3.24 \times$\\ $(2.24 \times)$}\\
% \noalign{\hrule height 0.75pt}
% \end{tabular}
% \label{tab:YOLOv3-tiny}
% \end{table}

%--------------------
% trade-off curves
%--------------------

%--------------------------------
%           Section 5
%--------------------------------
\section{Experimental Results}
\label{sec:results}
%\subsection{Experiment Setups}
% The proposed higher-order Tucker compression method is compared with the compression methods based on CP-decomposition \cite{Lebedev2014SpeedingupCN} and Tucker-$2$ decomposition \cite{Kim2016CompressionOD} on three well-known DNN architectures, namely, VGG-$16$ \cite{simonyan2014very}, AlexNet \cite{krizhevsky2012imagenet} and YOLOv$3$-tiny \cite{redmon2018yolov3}. VGG-16 and AlexNet are trained on \textit{CIFAR-10} \cite{krizhevsky2009learning}, while \textit{COCO}  \cite{lin2014microsoft} is the dataset for YOLOv3-tiny.

% The advantages of proposed higher-order Tucker compression are demonstrated by comparison with Tucker-2 method on three well-known CNN architectures, namely, VGG-$16$ \cite{simonyan2014very}, AlexNet \cite{krizhevsky2012imagenet} and YOLOv$3$-tiny \cite{redmon2018yolov3}. 
% The initialization environment is set as PyTorch for coding and NVIDIA GTX-1080Ti for hardware realization.
% Benchmarking is made on \textit{CIFAR-10} \cite{krizhevsky2009learning} (for VGG-16 and AlexNet) and \textit{COCO}  \cite{lin2014microsoft} (for YOLOv3-tiny).
% VGG-16 and AlexNet are trained on \textit{CIFAR-10} \cite{krizhevsky2009learning}, while \textit{COCO}  \cite{lin2014microsoft} is the dataset for YOLOv3-tiny. 
% CP decomposition method can only compress one or several layers, selecting ranks manually. At the setup stage, we use CP decomposition to compress all $12$ CONV layers but the first layer of VGG-16 as a preliminary result to see its performance when compressing as much CONV layers as possible. After fine-tuning, the testing accuracy is $10.07\%$, it is relatively low. Thus, CP decomposition is not included in the experiments due to its poor performance when compressing almost all layers of a CNN. 
% It should be noted that only CONV layers are compressed in our experiments.
The proposed higher-order Tucker compression method is compared with Tucker-2 decomposition~\cite{Kim2016CompressionOD} on three popular DNN architectures, namely, VGG-$16$~\cite{simonyan2014very}, AlexNet~\cite{krizhevsky2012imagenet}, and YOLOv$3$-tiny~\cite{redmon2018yolov3}.
All neural networks are implemented with PyTorch~\cite{paszke2017automatic}, and experiments are run on an NVIDIA GeForce GTX1080 Ti Graphics Card with $11$ GB frame buffer.
We use as a benchmark \textit{CIFAR-10}~\cite{krizhevsky2009learning} for VGG-16 and AlexNet, and \textit{COCO}~\cite{lin2014microsoft} for YOLOv3-tiny.
Note that we only compress CONV layers in all our experiments.

\setlength{\tabcolsep}{5mm}{
\begin{table}[t!]
\centering
\scriptsize
\caption{The accuracy and compression comparison among several realizations.}
\begin{tabular}{cccc}
\noalign{\hrule height 0.75pt}
& VGG-16 & AlexNet & YOLOv3-tiny  \\
\hline
Original & \tabincell{c}{$15$M\\ $(92.79\%)$}  & \tabincell{c}{$2446$K\\ $(90.86\%)$} & \tabincell{c}{$8333$K\\ (mAP$=31.3$)}\\
\hline
Tucker-2 & \tabincell{c}{$2507$K\\ $(92.01\%)$} & \tabincell{c}{$520$K\\ $(90.29\%)$} & \tabincell{c}{$5736$K\\ (mAP$=28.73$)}\\
\hline
HOTCAKE & \tabincell{c}{$1835$K\\ $(84.37\%)$} & \tabincell{c}{$261$K\\ $(83.17\%)$} & \tabincell{c}{$2566$K\\ (mAP$=25.58$)}\\
\hline
\tabincell{c}{Compression\\ Ratio} & \tabincell{c}{$8.02 \times$\\ $(1.37 \times)$} & \tabincell{c}{$9.37 \times$\\ $(1.99 \times)$} & \tabincell{c}{$3.24 \times$\\ $(2.24 \times)$}\\
\noalign{\hrule height 0.75pt}
\end{tabular}
\label{tab:3models}
\end{table}}

\setlength{\tabcolsep}{2.5mm}{
\begin{table*}[t!]
\caption{VGG-16 contains $13$ convolutional layers. And the first layer only contains $3$ input channels, thus only CONV2 to CONV13 are compressed. This table shows the \#params of each layer after being compressed by Tucker-2 and HOTCAKE, respectively, and the compression ratios of HOTCAKE vs original (and vs Tucker-2). For layers 2 to 4, HOTCAKE does not break the input channel to reach higher compression ratios, since the \#params is already very small after Tucker-2 decomposition.}
\scriptsize
\centering
\begin{tabular}{ccccccccccccc}
\noalign{\hrule height 0.75pt}
CONV layer& 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 \\
\hline
\tabincell{c}{Original\\ $(92.79\%)$}& $37$K & $74$K & $148$K & $295$K & $590$K & $590$K & $1180$K & $2360$K & $2360$K & $2360$K & $2360$K & $2360$K \\
\hline
\tabincell{c}{Tucker-2\\ $(92.01\%)$} & $4$K & $9$K & $18$K & $93$K & $157$K & $141$K & $251$K & $571$K & $295$K & $350$K & $386$K & $232$K \\
\hline
\tabincell{c}{HOTCAKE\\ $(84.37\%)$} & $4$K & $9$K & $18$K & $76$K & $107$K & $102$K & $180$K & $435$K & $214$K & $244$K & $273$K & $167$K \\
\hline
\tabincell{c}{Compression\\ Ratio} & -- & -- & -- & \tabincell{c}{$3.88 \times$\\ $(1.23 \times)$} & \tabincell{c}{$5.51 \times$\\ $(1.46 \times)$} & \tabincell{c}{$5.78 \times$\\ $(1.38 \times)$} & \tabincell{c}{$6.34 \times$\\ $(1.35 \times)$} & \tabincell{c}{$5.43 \times$\\ $(1.31 \times)$} & \tabincell{c}{$11.03 \times$\\ $(1.38 \times)$} & \tabincell{c}{$9.67 \times$\\ $(1.43 \times)$} & \tabincell{c}{$8.64 \times$\\ $(1.41 \times)$} & \tabincell{c}{$14.13 \times$\\ $(1.39 \times)$} \\
\noalign{\hrule height 0.75pt}
\end{tabular}
\label{tab:VGG-16}
\end{table*}}

\setlength{\tabcolsep}{3mm}{
\begin{table}[t]
\caption{Layer-wise evaluation on MTCNN by accuracy, compression, and \#params.}
%\caption{Layer-wise analysis of MTCNN and MTCNN's performance after being compressed by HOTCAKE.}
\centering
\scriptsize
%----------------------
% MTCNN
%----------------------
\begin{tabular}{ccccc}
\noalign{\hrule height 0.75pt}
CONV layer & 2 & 3 & 4 & Total\\
\hline
Original & $18$K & $37$K & $33$K & $88$K\\
HOTCAKE & $4$K & $8$K & $11$K & $23$K\\
\tabincell{c}{Compression\\ Ratio} & $ 4.5\times$ & $4.63\times $ & $3\times $ & $3.83\times $\\
\noalign{\hrule height 0.75pt}
Loss & Detection & \tabincell{c}{Bounding\\ Box} & Landmarks & Total\\
\hline
\tabincell{c}{Original\\ $(95.36\%)$} & $0.648$ & $0.0137$ & $0.0107$ & $0.546$ \\
\hline
\tabincell{c}{HOTCAKE\\ $(94.42\%)$} & $0.686$ & $0.0175$ & $0.0128$ & $0.569$\\
\noalign{\hrule height 0.75pt} 
\end{tabular}
\label{tab:MTCNN_Compress}
\end{table}}

As a preliminary result, we use CP decomposition to compress all but the first CONV layers of VGG-16, yielding a poor test accuracy of $10.07\%$ even after fine-tuning.
Therefore we do not include CP decomposition in the experiments due to its poor ability to perform deep compression on DNNs.


%--------------------------------
% VGG-16, AlexNet and YOLOv3-tiny
%--------------------------------
\subsection{Overall Results on VGG-16, AlexNet, and YOLOv3-tiny}
Table~\ref{tab:3models} summarizes results for the three CNNs.
In all rows but the last, each entry denotes the total number of parameters in the CONV layers (that are to be compressed), while the numbers in brackets are the post-fine-tuning model performance.
For YOLOv3-tiny, mAP stands for mean average precision, and the larger the better. Compression ratios to the original model are computed by  $\frac{\#params_{Original}}{\#params_{HOTCAKE}}$, and the HOTCAKE-to-(Tucker-2) ratios are in brackets.
% The number of parameters is the sum of parameters from CONV layers that are being compressed, not the total parameters of the CNN. The percentages in brackets are testing accuracy after fine-tuning. 
% For YOLOv3-tiny, mAP is the abbreviation of mean average precision, the larger the better.
% In the column where the table describes the compression ratio, the above ones are the ratio of $\frac{\#params_{Original}}{\#params_{HOTCAKE}}$, comparing model compressed by HOTCAKE with the original model. And the percentages in brackets are the ratio of $\frac{\#params_{Tucker-2}}{\#params_{HOTCAKE}}$, comparing the compression ability between Tucker-2 and HOTCAKE. 

It is demonstrated that the proposed HOTCAKE achieves a much higher compression ratio on all three models with a tolerable accuracy drop. 
For VGG-16 with totally 13 CONV layers, we compress all CONV layers except the first one, since its input channel number is only $3$.
On VGG-16, HOTCAKE gets $1.37\times$ higher compression ratio than Tucker-2, with accuracy dropping from $92.01\%$ to $84.37\%$.
For AlexNet (last $4$ of the $5$ CONV layers got compressed due to the same reason as for VGG-16), HOTCAKE is able to reach a $1.99 \times$ higher compression rate than Tucker-2, with an accuracy drop of $7.12\%$ from $90.29\%$ to $83.17\%$.
As for YOLOv3-tiny (except the first layer and the $1 \times 1$ CONV layers, we compress the remaining $6$ CONV layers), HOTCAKE gets $2.24 \times$ higher compression ratio, with mAP decreasing from $28.73$ to $25.58$. 

It is worth mentioning that pre-trained weights are a good initialization for both Tucker-2 and HOTCAKE.
If we keep the same model structure (layer dimension, etc.) and initialize the weights randomly, the accuracy cannot be recovered to an acceptable level even after adequate retraining ($50$ epochs in our experiment).

%Here we do not compare HOTCAKE with other pruning or quantization compression methods, as our proposed HOTCAKE is orthogonal to other compression techniques.
% For VGG-16, the number of params decreases $1.37 \times$ compared with Tucker-2, and that is $8.02 \times$ compression compared with the original model. The accuracy decrease $7.64\%$ from $92.01\%$ to $84.37\%$. As for AlexNet, the number of params is reduced by HOTCAKE for $9.37 \times$, and compared with Tucker-2, that is $1.37 \times$ compression. And the accuracy drops from $90.29\%$ to $83.17\%$. For YOLOv3-tiny, compared with original and Tucker-2, the compression reaches $3.24 \times$ and $2.24 \times$ respectively. And mAP changes from  $28.73$ to $25.58$. 

%------------------
% trade-off curves
%------------------


% \begin{table}[t]
% \caption{The first CONV layer of AlexNet only contains 3 input channels, thus we compress CONV layer 2 to 5.  }
% \scriptsize
% \centering
% \begin{tabular}{cccccc}
% \noalign{\hrule height 0.75pt}
% CONV layer & 2 & 3 & 4 & 5 & Total  \\
% \hline
% \tabincell{c}{Original\\ $(90.86\%)$} & $3. 07$K & $664$K & $885$K & $590$K & $2446$K\\
% \hline
% \tabincell{c}{Tucker-2\\ $(90.29\%)$} & $127$K & $197$K & $124$K & $71$K & $520$K \\
% \hline
% \tabincell{c}{HOTCAKE\\ $(83.17\%)$}& $56$K & $120$K & $51$K & $34$K & $261$K \\
% \hline
% \tabincell{c}{Compression\\ Ratio} & \tabincell{c}{$5.48 \times$\\ $(2.27 \times)$} & \tabincell{c}{$5.53 \times$\\ $(1.64 \times)$} & \tabincell{c}{$7.14 \times$\\ $(2.43 \times)$} & \tabincell{c}{$17.35 \times$\\ $(2.09 \times)$} & \tabincell{c}{$9.37 \times$\\ $(1.99 \times)$}\\
% \noalign{\hrule height 0.75pt}
% \end{tabular}
% \label{tab:AlexNet}
% \end{table}


%--------------------------------
%       Trade Off Curves
%--------------------------------
\subsection{Trade-off between Compression Ratio and Model Performance}
A trade-off exists between compression ratio and model performance.
Curves in Fig.~\ref{fig:TradeOffCurve} confirm such trade-off on the three models above.
According to the figure, a higher compression rate comes with a poorer testing accuracy.

\begin{figure*}[t] 
\begin{center}
\includegraphics[width=1\textwidth]{Figures/tradeoff.png}
\end{center}
\caption{Trade-off curves of VGG-16, AlexNet and YOLOv3-tiny.}
\label{fig:TradeOffCurve}
\end{figure*}

We noticed that by compressing layers in different orders, the obtainable model performance may vary.
Table~\ref{tab:VGG-16} shows the layer-wise statistics of VGG-16.
With the provided compression ratios by Tucker-2, we may arrange the compression order accordingly.
The orange curve in Fig.~\ref{fig:TradeOffCurve} shows how accuracy drops when compressing layers in the descending order of layer compression ratios.
As a quick example, if we are compressing VGG-16 on two of its CONV layers, CONV$6$ and CONV$11$ stand out since they have the highest compression ratios.
Note that with this order, the accuracy drops more slowly compared with compressing by layers sequentially. Therefore, with a pre-compressed model given, HOTCAKE is able to yield a specific compression order to reach a better balance between compression and performance.
% select specific layers to compress to get higher compression ratio with an acceptable decrease of accuracy.

% it is obvious that compressing layers having a large compression ratio first leads to smaller accuracy drop. Therefore, it is possible to select which layers to compress without using HOTCAKE to compress all of them, e.g. for VGG-16 (Table~\ref{tab:VGG-16} shows layer-wise analysis), when compared with Tucker-2, CONV2 has the highest compression ratio, followed by CONV11, CONV12, CONV13, etc.. By selecting layers in this order, a flexible trade-off between compression ratio and testing accuracy can be done.



%--------------------------------
%   Higher Compression Ratio
%-------------------------------
\subsection{Towards Higher Compression Ratio without Optimal Rank Selection}
We demonstrate the effectiveness of HOTCAKE when a higher compression ratio is expected. The compression ratio is determined by the ranks selected by VBMF.
We take AlexNet as an example, setting Tucker ranks manually to reach higher compression ratios, to examine the performance of both approaches.

According to the rank solution provided by VBMF, Tucker-2 decreases the number of parameters for $4.37 \times$ compared with the original AlexNet, and HOTCAKE decreases $9.37 \times$.
We then set ranks manually for Tucker-2 to reach the same compression ratio, obtaining an accuracy drop from $90.29\%$ to $81.39\%$, which is lower than that of HOTCAKE ($83.17\%$).
Next, we assign ranks for both Tucker-2 and HOTCAKE, to reach compression ratios at around $12 \times$, $14 \times$, and $16 \times$.
The results are illustrated in Fig.~\ref{fig:HigherRatio}, showing the advantage of HOTCAKE over Tucker-2 in deeper compressions. This also highlights the merit of HOTCAKE to search for highly compact CNNs.
% The two curves show HOTCAKE performs better than Tucker-2 when doing deeper compression. Thus, we highlight that HOTCAKE structure is better than Tucker-2 when searching for highly compacted CNNs. 

%----------------------
%        MTCNN
%----------------------
\subsection{Experiment on MTCNN}
We also tested the proposed higher order Tucker compression method on several lightweight CNNs, which is aiming to show that our proposed method can still remove the redundancy on an intentionally designed compact model. The first model we apply our method on is called MTCNN~\cite{7553523}, which is designed for human face detection. Considering the real time performance, the authors of~\cite{7553523} demonstrated a cascaded CNNs framework, while each build-in CNN is designed to be lightweight deliberately. Specifically, MTCNN contains three cascaded neural networks called Proposal Network (P-Net), Refinement Network (R-Net) and Output Network (O-Net).
O-Net is the biggest among the three, but it is still relatively small, containing $4$ CONV layers with the kernel tensor of $\ten{K}^{(1)} \in \mathbb{R}^{3 \times 3 \times 3 \times 32}$, $\ten{K}^{(2)} \in \mathbb{R}^{3 \times 3 \times 32 \times 64}$, $\ten{K}^{(3)} \in \mathbb{R}^{3 \times 3 \times 64 \times 64}$, and $\ten{K}^{(4)} \in \mathbb{R}^{3 \times 3 \times 64 \times 128}$, respectively. The datasets used in this task are \textit{WIDER FACE} \cite{yang2016wider} and \textit{CNN for Facial Point} \cite{sun2013deep}.


We compressed all CONV layers except the first one since its input channel dimension is only $3$. Table~\ref{tab:MTCNN_Compress} shows an overview of the results of compressed MTCNN. MTCNN contains three tasks, viz., human faces classification, detection, and landmark location.
The percentage in brackets are classification accuracy of human faces. The last two rows of the table list the loss of different tasks, where total loss is the weighted sum of all three tasks' loss.
Compared with the original MTCNN, the compression ratios of each CONV layer are $4.5 \times $, $4.63 \times $, and $3 \times $, respectively.
As for the performance, the face classification accuracy and mean error rate of face alignment both decrease within $1\%$.
The gaps between the loss of three tasks before and after being HOTCAKE compression are all quite small.
With the successful application on MTCNN, we argue that our proposed compression scheme can handle even the already-tiny models.
% In this subsection, we just compare Tucker-2 with the original model to claim that our proposed HOTCAKE can deal with a relatively small model.

%-------------------------
% Higher Compression Ratio
%-------------------------
\begin{figure}[t] 
\begin{center}
\includegraphics[width=0.45\textwidth]{Figures/alexnet.png}
\end{center}
% \caption{This figure shows how accuracy drops when Tucker ranks are not selected by VBMF as higher compression ratio is in the priority.}
\caption{Accuracy v.s. compression on Cifar-10.}
%\caption{The two curves here show the trend of decreasing accuracy when higher compression ratio is expected.}
\label{fig:HigherRatio}
\end{figure}

\subsection{Experiment on SimpNet}
Another lightweight CNN we compressed is SimpNet~\cite{hasanpour2018towards}, which is designed by following some simple but crucial principles. Compared with the CNNs designed ad-hoc, SimpNet enjoys the properties of allowing granular tuning and automated architecture design approaches. Due to the efficient and compact architecture, SimpNet can potentially achieve superior performance in many real-life scenarios, especially when employing it in  mobile devices, embeded systems and deeping learning application at the edge. Thought having tens times less of network parameters than some deeper and more complex CNNs, SimpNet still obtains state-of-the-art results on several standard datasets.





==> template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering
